The effect of space charge on photon-enhanced thermionic emission in the presence of the bidirectional discharge

The bidirectional space charge effects in photon-enhanced thermionic emission (PETE) devices are investigated systematically. First, we precisely determine the carrier concentrations and cathode temperatures by taking into account the electron recycling effect, energy balance constraints, and space charge effects arising from the concurrent discharge of the cathode and anode. Next, we analyze the impact of critical parameters, including anode properties and operating conditions, on the space charge barrier distribution and the overall performance of the device. The results demonstrate that the impact of reverse discharge on the net current becomes more pronounced when the PETE device operates at high anode temperatures, low anode work functions, and with a moderate solar concentration ratio and gap width. This discovery not only deepens our understanding of the bidirectional space charge effect, but also provides valuable guidance for the future optimization of PETE device performance.

==> PETE_SCBD_cover_letter.tex <==
Dear Editor:
The manuscript entitled “The effect of space charge on photon-enhanced thermionic emission in the presence of the bidirectional discharge” is being submitted to Physical Review Applied by Xinqiao Lin, Ousi Pan, Zhimin Yang, Yanchao Zhang, Jincan Chen, and Shanhe Su. The reason that the proposed work may be of particular interest to the readers of Physical Review Applied are as follows:
Photon-enhanced thermionic emission is a solar energy conversion technique that aims to integrate photon and thermal processes into a single mechanism. This study aims to investigate the effects of space charge on photon-enhanced thermionic emission. The Child-Langmuir space charge theory has been applied here, taking into account the effects of bidirectional discharge. The potential diagram, which is proportional to the electrostatic potential, is derived from the solution to Poisson’s equation. The results show that the effect of reverse discharge on the net current is more significant when the PETE device operates at high anode temperatures, low anode work functions, and with moderate solar concentration ratios and gap widths. This discovery not only enhances our understanding of the bidirectional space charge effect but also offers valuable insights for optimizing the performance of PETE devices in the future.
The possible reviewers of our manuscript are listed as follows:
1. Prof. Bjarne Andresen, Niels Bohr Institute, University of Copenhagen, Denmark, andresen@fys.ku.dk;
2. Prof. S.K. Tyagi, School of Infrastructure Technology and Resource Management, Shri Mata Vaishno Devi University, India, sudhirtyagi@yahoo.com;
3. Prof. Binhong Lin, College of Information Science and Engineering, Huaqiao University, China, bhlin@hqu.edu.cn.

    Your editorial assistance is much appreciated.

Sincerely yours,
Xinqiao Lin

